Unitary Expressions: A Necessary Abstraction for Extensible Quantum Programming Languages and Systems

Quantum gates are the fundamental instructions of digital quantum computers. Current programming languages, systems, and software development toolkits identify these operational gates by their titles, which requires a shared understanding of their meanings. However, in the continuously developing software ecosystem surrounding quantum computing -- spanning high-level programming systems to low-level control stacks -- this identification process is often error-prone, challenging to debug, maintenance-heavy, and resistant to change. In this paper, we propose replacing this nominal gate representation with a functional one. We introduce the OpenQudit system for describing, parsing, optimizing, analyzing, and utilizing programs comprising gates described as symbolic unitary expressions. As part of this effort, we design the Qudit Gate Language (QGL), a unitary-specific expression language, and implement a differentiating just-in-time compiler in OpenQudit towards embedding this language in quantum programming languages and systems. Additionally, we have precisely designed and implemented the Qudit Virtual Machine (QVM) to evaluate quantum programs and their gradients efficiently. This evaluation is performed millions of times during the compilation of quantum programs. Our QVM can compute gradients approximately ten times faster than current leading numerical quantum compilation frameworks in the most common use cases. Altogether, the OpenQudit system is envisioned to (1) support many-level or qudit-based quantum systems, (2) enable the safe composition of program transformation tools, (3) accelerate circuit optimizers and transpilers, (4) enable compiler extensibility, and (5) provide a productive, simple-to-use interface to quantum practitioners.

==> sections/related.tex <==
\section{Related Works}
\label{sec:related}

\subsection{Quartz}
Quartz~\cite{quartz} is a superoptimizing quantum compiler that, given a gate set, first discovers symbolic rewrite rules over the gate set and then applies the rules over a larger circuit to reduce the program instruction count. Rewrite rules are found by enumerating all subcircuits to a specified qubit, gate, and parameter count, placing them in equivalence classes by verifying equality with a representative symbolic circuit. Equality verification reduces the problem to quantifier-free nonlinear real arithmetic by exhaustive applications of trigonometric identities and introducing fresh variables, at which point Quartz applies an SMT solver. It can uncover thousands of rewritten rules at the cost of long runtimes. Unfortunately, Quartz requires user-specified rewrite rules to translate from one gate set to another and cannot optimize gate expressions toward JIT compilation or autodifferentiation.

\subsection{QUESO}
The QUESO~\cite{queso} tool finds probabilistic symbolic rewrite rules over subcircuits extremely quickly and applies them in a larger circuit toward optimizing overall gate counts with a beam search. Its efficiency arises by phrasing symbolic circuit equivalence as a polynomial identity testing (PIT) problem and then applying the Schwartz-Zippel lemma. This process determines equality with high confidence, albeit with a slight chance of producing an incorrect rule. QUESO cannot prove equivalence, even probabilistically, between two globally phase congruent symbolic circuits and, as such, finds fewer rules than the Quartz rule finder. Additionally, QUESO is not equipped to optimize an expression representation and JIT compile it. However, even with fewer rewrite rules discovered, the beam search rewrite application method is effective and competitive with TKET and Quartz.

\subsection{Numerical Quantum Compilers}
A class of quantum compilers and compilation algorithms work on numerical instantiation -- using a numerical optimizer to find the ``best'' arguments for parameterized quantum circuits given a concrete target -- to effectively resynthesis concrete circuits. Here, concrete circuits are mapped to others that are better according to the algorithm's objective function. Typically, this is the gate count, but it can also be optimized for specific gate usage and other circuit characteristics. The optimizations uncovered can outperform rule-based peephole techniques alone since they work on concrete subcircuits and, as a result, uncover specific rewrite rules for a given instantiated circuit and scale to much larger sizes. These algorithms can effectively translate programs between gate sets but must understand how to evaluate each gate and its gradients before operation. Additionally, their scalability depends on efficient implementations, often requiring low-level hand-optimization and analytic differentiation. For many algorithm designers and quantum computer users, these barriers can slow down adoption, especially regarding new and emerging gate sets and quantum technologies.
